Towards Better Evaluation for Dynamic Link Prediction

Despite the prevalence of recent success in learning from static graphs, learning from time-evolving graphs remains an open challenge. In this work, we design new, more stringent evaluation procedures for link prediction specific to dynamic graphs, which reflect real-world considerations, to better compare the strengths and weaknesses of methods. First, we create two visualization techniques to understand the reoccurring patterns of edges over time and show that many edges reoccur at later time steps. Based on this observation, we propose a pure memorization baseline called EdgeBank. EdgeBank achieves surprisingly strong performance across multiple settings because easy negative edges are often used in the current evaluation setting. To evaluate against more difficult negative edges, we introduce two more challenging negative sampling strategies that improve robustness and better match real-world applications. Lastly, we introduce six new dynamic graph datasets from a diverse set of domains missing from current benchmarks, providing new challenges and opportunities for future research. Our code repository is accessible at https://github.com/fpour/DGB.git.

==> content/030_preliminary.tex <==
% \section{Preliminaries}
\section{Related Work}

==> content/080_checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{Please see Appendix~\ref{app:limit} for discussion about the limitations of our work.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{Our work focus on evaluating existing dynamic link predictions methods; thus, it is unclear if any direct negative societal impact would occur as a result. However, we discuss potential negative impacts in Appendix~\ref{app:impact} for dynamic link prediction task in general.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{We conform to the ethics guidelines.}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Our code and data can be found on the project repository on \href{https://github.com/fpour/DGB.git}{github}. This is also mentioned in \textit{Reproducibility} part of Section \ref{sec:introduction}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{We report training details for reproducibility in Section~\ref{sec:experiments} and Appendix~\ref{app:hype}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We report error bars in Appendix~\ref{subsec:extended_results} for different settings and performance metrics. (Please note that since the standard deviations of the reported results are mostly within a small range, we reported them in the Appendix~\ref{subsec:extended_results} to improve readability of Fig. \ref{fig:abs_perf}.)}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{We report this information in Appendix~\ref{subsec:computing_resources}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{Yes, the assets are in MIT licence or Apache License 2.0, noted in Appendix~\ref{subsec:baseline_methods} and Section~\ref{subsec:datasets}.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We shared the link to  our github repository at~\url{https://github.com/fpour/DGB.git}. The link to our datasets repository at \url{https://zenodo.org/record/7008205\#.Yv_a_3bMJPZ}.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{None of our data contains personally identifiable information and they are already licensed and open sourced. Please see Appendix~\ref{subsec:datasets}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

==> content/arXiv/101_app_standard_rnd.tex <==
\subsection{Standard Negative Sampling - rnd}



\begin{table*}
\label{tab:acc_thr_0.5_transductive_mean}
\caption{Accuracy Results.}
\resizebox{\linewidth}{!}{%
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.8978 & 0.9237 & 0.7652 & 0.5542 & 0.7744 & 0.8030 & 0.5703 & 0.8666 & 0.7536 & 0.8027 & 0.6290 & 0.6348	\\
		DyRep & 0.8678 & 0.9278 & 0.7536 & 0.5664 & 0.7495 & 0.8257 & 0.4618 & 0.8569 & 0.5651 & 0.6419 & 0.5888 & 0.6085	\\
		TGAT & 0.8791 & 0.9302 & 0.6124 & 0.5007 & 0.5908 & 0.7055 & 0.7329 & 0.8197 & 0.6617 & 0.7108 & 0.5601 & 0.5070	\\
		TGN & 0.9345 & 0.9435 & 0.8399 & 0.5146 & 0.7518 & 0.9101 & 0.7440 & 0.9289 & 0.6320 & 0.7835 & 0.6278 & 0.6828	\\
		CAWN & 0.7197 & 0.9912 & 0.6514 & 0.6425 & 0.5209 & 0.6173 & 0.9210 & 0.9632 & 0.8318 & 0.8083 & 0.8728 & 0.6709	\\
		\midrule
		ebank (RF) & 0.8282 & 0.8623 & 0.5265 & 0.7535 & 0.7451 & 0.8160 & 0.6864 & 0.8083 & 0.6059 & 0.5198 & 0.5997 & 0.5566	\\
		ebank (TWF) & 0.8709 & 0.9143 & 0.6086 & 0.8377 & 0.8705 & 0.6790 & 0.7619 & 0.8402 & 0.6414 & 0.6257 & 0.6665 & 0.6198	\\
		ebank (TWAR) & 0.7757 & 0.8701 & 0.5933 & 0.8173 & 0.8085 & 0.7633 & 0.6108 & 0.8155 & 0.4837 & 0.4954 & 0.6675 & 0.6297	\\
		ebank (UM) & 0.9078 & 0.9537 & 0.5484 & 0.8351 & 0.8536 & 0.5390 & 0.7730 & 0.9023 & 0.6015 & 0.5903 & 0.6214 & 0.5834	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:ap_inherent_transductive_mean}
\caption{AP Results.}
\resizebox{\linewidth}{!}{%
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.9473 & 0.9528 & 0.7798 & 0.6833 & 0.7762 & 0.7921 & 0.7516 & 0.9358 & 0.7469 & 0.7633 & 0.6374 & 0.6420	\\
		DyRep & 0.9470 & 0.9806 & 0.7984 & 0.7076 & 0.7953 & 0.8747 & 0.4622 & 0.9296 & 0.5821 & 0.6419 & 0.6099 & 0.6514	\\
		TGAT & 0.9539 & 0.9819 & 0.6064 & 0.5033 & 0.5888 & 0.7586 & 0.7838 & 0.8949 & 0.6830 & 0.6973 & 0.5805 & 0.5167	\\
		TGN & 0.9851 & 0.9873 & 0.9042 & 0.7183 & 0.8540 & 0.9345 & 0.8812 & 0.9766 & 0.6427 & 0.7700 & 0.6398 & 0.7079	\\
		CAWN & 0.9922 & 0.9999 & 0.7476 & 0.9801 & 0.9502 & 0.7169 & 0.9945 & 0.9990 & 0.9431 & 0.9748 & 0.9739 & 0.8184	\\
		\midrule
		ebank (RF) & 0.8271 & 0.8608 & 0.5178 & 0.7234 & 0.7310 & 0.7495 & 0.6824 & 0.8054 & 0.6105 & 0.5123 & 0.5662 & 0.5349	\\
		ebank (TWF) & 0.8694 & 0.9114 & 0.5797 & 0.7929 & 0.8353 & 0.6094 & 0.7568 & 0.8365 & 0.6455 & 0.5839 & 0.6018 & 0.5712	\\
		ebank (TWAR) & 0.7750 & 0.8682 & 0.5725 & 0.7835 & 0.7884 & 0.6813 & 0.6101 & 0.8126 & 0.5000 & 0.5029 & 0.6041 & 0.5849	\\
		ebank (UM) & 0.9037 & 0.9486 & 0.5291 & 0.7725 & 0.8037 & 0.5204 & 0.7620 & 0.8935 & 0.6046 & 0.5545 & 0.5697 & 0.5470	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}

\begin{table*}
\label{tab:au_pr_score_transductive_mean}
\caption{AU-PR Results.}
\resizebox{\linewidth}{!}{%
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.9463 & 0.9511 & 0.7779 & 0.6811 & 0.7601 & 0.7895 & 0.7486 & 0.9353 & 0.7452 & 0.7609 & 0.6194 & 0.6379	\\
		DyRep & 0.9458 & 0.9805 & 0.7960 & 0.7025 & 0.7762 & 0.8709 & 0.4535 & 0.9291 & 0.5798 & 0.6389 & 0.5922 & 0.6477	\\
		TGAT & 0.9537 & 0.9818 & 0.6030 & 0.6519 & 0.5858 & 0.7570 & 0.7828 & 0.8944 & 0.6803 & 0.6944 & 0.6281 & 0.5132	\\
		TGN & 0.9851 & 0.9873 & 0.9037 & 0.7166 & 0.8424 & 0.9339 & 0.8808 & 0.9765 & 0.6400 & 0.7678 & 0.6368 & 0.7056	\\
		CAWN & 0.9921 & 0.9999 & 0.7971 & 0.9797 & 0.9493 & 0.7191 & 0.9944 & 0.9994 & 0.9422 & 0.9744 & 0.9735 & 0.8155	\\
		\midrule
		ebank (RF) & 0.9129 & 0.9298 & 0.5867 & 0.8323 & 0.8313 & 0.8599 & 0.8339 & 0.9013 & 0.5349 & 0.5892 & 0.6751 & 0.6582	\\
		ebank (TWF) & 0.9341 & 0.9552 & 0.6990 & 0.8818 & 0.9026 & 0.8042 & 0.8736 & 0.9168 & 0.5821 & 0.7135 & 0.7882 & 0.7810	\\
		ebank (TWAR) & 0.8870 & 0.9334 & 0.6995 & 0.8750 & 0.8777 & 0.8394 & 0.8026 & 0.9049 & 0.2794 & 0.3478 & 0.7796 & 0.7700	\\
		ebank (UM) & 0.9509 & 0.9738 & 0.6397 & 0.8743 & 0.8850 & 0.7601 & 0.8720 & 0.9451 & 0.5990 & 0.7031 & 0.7794 & 0.7725	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}

\begin{table*}
\label{tab:auc_inherent_transductive_mean}
\caption{AU-ROC Results.}
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.9593 & 0.9725 & 0.8276 & 0.6904 & 0.8287 & 0.8615 & 0.8251 & 0.9456 & 0.8095 & 0.8404 & 0.6718 & 0.6668	\\
		DyRep & 0.9448 & 0.9802 & 0.8242 & 0.7065 & 0.8213 & 0.8966 & 0.4374 & 0.9397 & 0.6404 & 0.6997 & 0.6213 & 0.6765	\\
		TGAT & 0.9523 & 0.9811 & 0.6487 & 0.5010 & 0.6205 & 0.7791 & 0.8063 & 0.9003 & 0.7296 & 0.7654 & 0.5980 & 0.5144	\\
		TGN & 0.9845 & 0.9869 & 0.9182 & 0.7291 & 0.8717 & 0.9532 & 0.8786 & 0.9793 & 0.7064 & 0.8340 & 0.6801 & 0.7468	\\
		CAWN & 0.9891 & 0.9999 & 0.7119 & 0.9734 & 0.9327 & 0.6742 & 0.9922 & 0.9991 & 0.9215 & 0.9642 & 0.9621 & 0.7515	\\
		\midrule
		ebank (RF) & 0.8282 & 0.8623 & 0.5265 & 0.7535 & 0.7451 & 0.8160 & 0.6864 & 0.8083 & 0.6059 & 0.5198 & 0.5997 & 0.5566	\\
		ebank (TWF) & 0.8709 & 0.9143 & 0.6086 & 0.8377 & 0.8705 & 0.6790 & 0.7619 & 0.8402 & 0.6414 & 0.6257 & 0.6665 & 0.6198	\\
		ebank (TWAR) & 0.7757 & 0.8701 & 0.5933 & 0.8173 & 0.8085 & 0.7633 & 0.6108 & 0.8155 & 0.4837 & 0.4954 & 0.6675 & 0.6297	\\
		ebank (UM) & 0.9078 & 0.9537 & 0.5484 & 0.8351 & 0.8536 & 0.5390 & 0.7730 & 0.9023 & 0.6015 & 0.5903 & 0.6214 & 0.5834	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:f1_thr_0.5_transductive_mean}
\caption{F1-score Results.}
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.8963 & 0.9245 & 0.7779 & 0.6733 & 0.7930 & 0.8077 & 0.2903 & 0.8764 & 0.7753 & 0.8325 & 0.6827 & 0.6357	\\
		DyRep & 0.8652 & 0.9285 & 0.7716 & 0.6979 & 0.7725 & 0.8305 & 0.1565 & 0.8680 & 0.6813 & 0.6136 & 0.6014 & 0.6457	\\
		TGAT & 0.8786 & 0.9306 & 0.6688 & 0.6076 & 0.6647 & 0.7083 & 0.7697 & 0.8244 & 0.6325 & 0.7360 & 0.5363 & 0.4163	\\
		TGN & 0.9344 & 0.9437 & 0.8388 & 0.6733 & 0.7922 & 0.9114 & 0.7855 & 0.9287 & 0.7152 & 0.8097 & 0.6779 & 0.7129	\\
		CAWN & 0.8076 & 0.9883 & 0.7637 & 0.7506 & 0.6717 & 0.7449 & 0.9311 & 0.9740 & 0.7840 & 0.6419 & 0.8859 & 0.5315	\\
		\midrule
		ebank (RF) & 0.7905 & 0.8403 & 0.2537 & 0.6981 & 0.6484 & 0.8231 & 0.5404 & 0.7545 & 0.3088 & 0.2331 & 0.5518 & 0.4973	\\
		ebank (TWF) & 0.8507 & 0.9065 & 0.4714 & 0.8305 & 0.8602 & 0.7567 & 0.6873 & 0.8049 & 0.4187 & 0.5675 & 0.7370 & 0.7211	\\
		ebank (TWAR) & 0.7077 & 0.8508 & 0.3933 & 0.7951 & 0.7679 & 0.8080 & 0.3550 & 0.7671 & 0.0000 & 0.0220 & 0.7258 & 0.7062	\\
		ebank (UM) & 0.8982 & 0.9518 & 0.4877 & 0.8433 & 0.8524 & 0.6844 & 0.7114 & 0.8914 & 0.4429 & 0.6071 & 0.7203 & 0.7058	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:prec_thr_0.5_transductive_mean}
\caption{Precision Results.}
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.9051 & 0.9145 & 0.7385 & 0.5418 & 0.7268 & 0.7893 & 0.7379 & 0.8262 & 0.6890 & 0.7255 & 0.5900 & 0.5704	\\
		DyRep & 0.8775 & 0.9199 & 0.7221 & 0.5478 & 0.7125 & 0.8089 & 0.2961 & 0.8136 & 0.5342 & 0.6222 & 0.5654 & 0.5468	\\
		TGAT & 0.8819 & 0.9253 & 0.5847 & 0.5006 & 0.5625 & 0.6986 & 0.6768 & 0.8037 & 0.6321 & 0.6757 & 0.6384 & 0.6008	\\
		TGN & 0.9358 & 0.9417 & 0.8418 & 0.5079 & 0.6905 & 0.8982 & 0.6838 & 0.9299 & 0.5789 & 0.7219 & 0.5906 & 0.6496	\\
		CAWN & 0.7182 & 0.9958 & 0.6429 & 0.6438 & 0.5179 & 0.6173 & 0.9283 & 0.9621 & 0.8940 & 0.9832 & 0.8900 & 0.8438	\\
		\midrule
		ebank(RF) & 0.9965 & 0.9957 & 0.5916 & 0.8680 & 0.8979 & 0.7861 & 0.9772 & 0.9913 & 0.4341 & 0.5997 & 0.5743 & 0.5745	\\
		ebank (TWF) & 0.9957 & 0.9931 & 0.7211 & 0.8616 & 0.8811 & 0.6097 & 0.9797 & 0.9896 & 0.4609 & 0.6671 & 0.6088 & 0.5722	\\
		ebank (TWAR) & 0.9976 & 0.9947 & 0.7640 & 0.8876 & 0.9172 & 0.6830 & 0.9938 & 0.9912 & 0.0588 & 0.1860 & 0.6173 & 0.5763	\\
		ebank (UM) & 0.9898 & 0.9888 & 0.5625 & 0.8051 & 0.8274 & 0.5204 & 0.9586 & 0.9783 & 0.4762 & 0.5842 & 0.5716 & 0.5472	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:rec_thr_0.5_transductive_mean}
\caption{Recall Results.}
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.8891 & 0.9353 & 0.8255 & 0.9210 & 0.8832 & 0.8379 & 0.1900 & 0.9371 & 0.9047 & 0.9796 & 0.8217 & 0.7693	\\
		DyRep & 0.8551 & 0.9375 & 0.8335 & 0.9785 & 0.8642 & 0.8605 & 0.1115 & 0.9339 & 0.9448 & 0.6747 & 0.6679 & 0.8259	\\
		TGAT & 0.8768 & 0.9362 & 0.7827 & 0.8179 & 0.8195 & 0.7208 & 0.8933 & 0.8477 & 0.6641 & 0.8122 & 0.6934 & 0.5376	\\
		TGN & 0.9333 & 0.9459 & 0.8383 & 0.9993 & 0.9401 & 0.9264 & 0.9301 & 0.9289 & 0.9417 & 0.9279 & 0.8065 & 0.8227	\\
		CAWN & 0.9927 & 0.9901 & 0.9985 & 0.9853 & 0.9799 & 1.0000 & 0.9757 & 0.9986 & 0.8325 & 0.6429 & 0.9478 & 0.6051	\\
		\midrule
		ebank (RF) & 0.6588 & 0.7279 & 0.1636 & 0.5932 & 0.5294 & 0.8671 & 0.3814 & 0.6225 & 0.2714 & 0.1574 & 0.5516 & 0.4839	\\
		ebank (TWF) & 0.7451 & 0.8344 & 0.3540 & 0.8041 & 0.8484 & 0.9973 & 0.5349 & 0.6881 & 0.4067 & 0.5198 & 0.9353 & 0.9797	\\
		ebank (TWAR) & 0.5526 & 0.7442 & 0.2702 & 0.7248 & 0.6764 & 0.9915 & 0.2228 & 0.6371 & 0.0000 & 0.0190 & 0.8836 & 0.9275	\\
		ebank (UM) & 0.8241 & 0.9178 & 0.4340 & 0.8870 & 0.8854 & 0.9997 & 0.5706 & 0.8239 & 0.4438 & 0.6440 & 0.9744 & 0.9956	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}





==> content/arXiv/102_app_hist_nre.tex.tex <==
\subsection{Adversarial Negative Edge Sampling: Hist-NRE}


\begin{table*}
\label{tab:acc_thr_0.5_transductive_mean}
\caption{Accuracy Results. \textcolor{red}{(hist-nre)}}
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.6447 & 0.6109 & 0.7358 & 0.5555 & 0.6137 & 0.7793 & 0.5209 & 0.5597 & 0.6096 & 0.6731 & 0.5912 & 0.6607	\\
		DyRep & 0.6545 & 0.6090 & 0.7526 & 0.5492 & 0.6597 & 0.8624 & 0.4477 & 0.5524 & 0.5786 & 0.6348 & 0.5642 & 0.6287	\\
		TGAT & 0.5860 & 0.5907 & 0.5694 & 0.4990 & 0.5216 & 0.7072 & 0.5215 & 0.5698 & 0.6519 & 0.7005 & 0.5199 & 0.5022	\\
		TGN & 0.5796 & 0.6002 & 0.7716 & 0.5012 & 0.6242 & 0.8613 & 0.5455 & 0.5542 & 0.6047 & 0.7271 & 0.5810 & 0.6938	\\
		CAWN & 0.4979 & 0.6175 & 0.4992 & 0.4995 & 0.4904 & 0.5368 & 0.5223 & 0.5074 & 0.7474 & 0.8041 & 0.5213 & 0.6084	\\
		\midrule
		ebank (RF) & 0.7727 & 0.7853 & 0.4618 & 0.6922 & 0.6903 & 0.8586 & 0.5614 & 0.7461 & 0.5259 & 0.4672 & 0.7208 & 0.6426	\\
		ebank (TWF) & 0.7706 & 0.7704 & 0.6018 & 0.7573 & 0.7527 & 0.7990 & 0.6934 & 0.7097 & 0.6284 & 0.6763 & 0.8097 & 0.7871	\\
		ebank (TWAR) & 0.7505 & 0.7859 & 0.6190 & 0.7816 & 0.7980 & 0.8678 & 0.6097 & 0.7237 & 0.4991 & 0.5072 & 0.8655 & 0.8959	\\
		ebank (UM) & 0.4915 & 0.5147 & 0.2916 & 0.5013 & 0.4803 & 0.5491 & 0.3507 & 0.4707 & 0.2737 & 0.3885 & 0.5361 & 0.5285	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:ap_inherent_transductive_mean}
\caption{AP Results. \textcolor{red}{(hist-nre)} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.7684 & 0.7715 & 0.6972 & 0.6824 & 0.5562 & 0.7266 & 0.6236 & 0.6451 & 0.4346 & 0.4509 & 0.5596 & 0.6577	\\
		DyRep & 0.8076 & 0.7886 & 0.7434 & 0.7078 & 0.7144 & 0.9324 & 0.4530 & 0.6259 & 0.5736 & 0.6255 & 0.5807 & 0.6370	\\
		TGAT & 0.7608 & 0.7707 & 0.5905 & 0.4992 & 0.5287 & 0.7699 & 0.6078 & 0.6505 & 0.6669 & 0.6299 & 0.5088 & 0.5114	\\
		TGN & 0.8799 & 0.8112 & 0.8402 & 0.7636 & 0.7227 & 0.9459 & 0.7640 & 0.6404 & 0.5604 & 0.5621 & 0.5710 & 0.6704	\\
		CAWN & 0.8879 & 0.8890 & 0.6617 & 0.5615 & 0.6324 & 0.6412 & 0.7902 & 0.6318 & 0.8971 & 0.8174 & 0.7206 & 0.7468	\\
		\midrule
		ebank (RF) & 0.7334 & 0.7352 & 0.4871 & 0.6443 & 0.6556 & 0.8064 & 0.5399 & 0.7050 & 0.5660 & 0.4944 & 0.6904 & 0.6096	\\
		ebanK (TWF) & 0.7133 & 0.7006 & 0.5729 & 0.6901 & 0.6834 & 0.7139 & 0.6526 & 0.6529 & 0.6374 & 0.6349 & 0.7322 & 0.7055	\\
		ebank (TWAR) & 0.7296 & 0.7328 & 0.6071 & 0.7313 & 0.7683 & 0.7941 & 0.6082 & 0.6743 & 0.5000 & 0.5058 & 0.8123 & 0.8484	\\
		ebank (UM) & 0.4964 & 0.5076 & 0.4314 & 0.5012 & 0.4953 & 0.5259 & 0.4430 & 0.4872 & 0.4797 & 0.4556 & 0.5189 & 0.5147	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:au_pr_score_transductive_mean}
\caption{AU-PR Results. \textcolor{red}{(hist-nre)} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.7654 & 0.7691 & 0.6941 & 0.6803 & 0.5401 & 0.7236 & 0.6207 & 0.6421 & 0.4328 & 0.4491 & 0.5384 & 0.6535	\\
		DyRep & 0.8009 & 0.7866 & 0.7388 & 0.7041 & 0.6911 & 0.9313 & 0.4447 & 0.6233 & 0.5713 & 0.6226 & 0.5613 & 0.6332	\\
		TGAT & 0.7597 & 0.7691 & 0.5876 & 0.6477 & 0.5255 & 0.7686 & 0.6063 & 0.6479 & 0.6641 & 0.6267 & 0.5561 & 0.5079	\\
		TGN & 0.8796 & 0.8099 & 0.8395 & 0.7624 & 0.7087 & 0.9454 & 0.7633 & 0.6375 & 0.5575 & 0.5597 & 0.5678 & 0.6678	\\
		CAWN & 0.8862 & 0.8919 & 0.7581 & 0.5659 & 0.6220 & 0.6387 & 0.7822 & 0.7882 & 0.8954 & 0.8149 & 0.7162 & 0.7430	\\
		\midrule
		ebank (RF) & 0.8408 & 0.8433 & 0.4900 & 0.7648 & 0.7526 & 0.8926 & 0.6386 & 0.8158 & 0.4783 & 0.4806 & 0.7792 & 0.7082	\\
		ebank (TWF) & 0.8286 & 0.8286 & 0.6873 & 0.8182 & 0.8144 & 0.8566 & 0.7736 & 0.7794 & 0.5747 & 0.7578 & 0.8579 & 0.8496	\\
		ebank (TWAR) & 0.8449 & 0.8423 & 0.7634 & 0.8392 & 0.8648 & 0.8963 & 0.7977 & 0.7916 & 0.7402 & 0.7509 & 0.8972 & 0.9152	\\
		ebank (UM) & 0.7032 & 0.7335 & 0.5264 & 0.7219 & 0.7133 & 0.7629 & 0.5897 & 0.6967 & 0.4962 & 0.6225 & 0.7532 & 0.7563	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:auc_inherent_transductive_mean}
\caption{AU-ROC Results. \textcolor{red}{(hist-nre)} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.7878 & 0.7873 & 0.7699 & 0.6910 & 0.6220 & 0.8276 & 0.7114 & 0.6731 & 0.4534 & 0.4948 & 0.6024 & 0.7042	\\
		DyRep & 0.7880 & 0.7954 & 0.7999 & 0.7011 & 0.7398 & 0.9328 & 0.4389 & 0.6577 & 0.6403 & 0.6912 & 0.5887 & 0.6772	\\
		TGAT & 0.7378 & 0.7763 & 0.6076 & 0.4978 & 0.5333 & 0.7810 & 0.5745 & 0.6545 & 0.7131 & 0.7276 & 0.5176 & 0.5080	\\
		TGN & 0.8398 & 0.8119 & 0.8522 & 0.7693 & 0.7506 & 0.9465 & 0.7193 & 0.6628 & 0.6338 & 0.6807 & 0.6058 & 0.7295	\\
		CAWN & 0.8442 & 0.8545 & 0.5968 & 0.4016 & 0.5069 & 0.5640 & 0.7291 & 0.6102 & 0.8598 & 0.7370 & 0.6033 & 0.6464	\\
		\midrule
		ebank (RF) & 0.7727 & 0.7853 & 0.4618 & 0.6922 & 0.6903 & 0.8586 & 0.5614 & 0.7461 & 0.5259 & 0.4672 & 0.7208 & 0.6426	\\
		ebank (TWF) & 0.7706 & 0.7704 & 0.6018 & 0.7573 & 0.7527 & 0.7990 & 0.6934 & 0.7097 & 0.6284 & 0.6763 & 0.8097 & 0.7871	\\
		ebank (TWAR) & 0.7505 & 0.7859 & 0.6190 & 0.7816 & 0.7980 & 0.8678 & 0.6097 & 0.7237 & 0.4991 & 0.5072 & 0.8655 & 0.8959	\\
		ebank (UM) & 0.4915 & 0.5147 & 0.2916 & 0.5013 & 0.4803 & 0.5491 & 0.3507 & 0.4707 & 0.2737 & 0.3885 & 0.5361 & 0.5285	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:f1_thr_0.5_transductive_mean}
\caption{F1-score Results. \textcolor{red}{(hist-nre)} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.7142 & 0.7063 & 0.7569 & 0.6725 & 0.6919 & 0.7896 & 0.2702 & 0.6802 & 0.6898 & 0.7497 & 0.6622 & 0.6538	\\
		DyRep & 0.7116 & 0.7057 & 0.7702 & 0.6847 & 0.7132 & 0.8605 & 0.1524 & 0.6758 & 0.6878 & 0.6118 & 0.5885 & 0.6575	\\
		TGAT & 0.6794 & 0.6958 & 0.6450 & 0.6068 & 0.6292 & 0.7094 & 0.6508 & 0.6630 & 0.6253 & 0.7285 & 0.5160 & 0.4143	\\
		TGN & 0.6894 & 0.7030 & 0.7853 & 0.6671 & 0.7132 & 0.8698 & 0.6713 & 0.6755 & 0.6996 & 0.7712 & 0.6524 & 0.7198	\\
		CAWN & 0.6627 & 0.7389 & 0.6656 & 0.6589 & 0.6539 & 0.6912 & 0.6709 & 0.6710 & 0.7382 & 0.6396 & 0.6620 & 0.5028	\\
		\midrule
		ebank (RF) & 0.7411 & 0.7718 & 0.2309 & 0.6505 & 0.6073 & 0.8577 & 0.4589 & 0.7016 & 0.2825 & 0.2206 & 0.6357 & 0.5538	\\
		ebank (TWF) & 0.7633 & 0.7841 & 0.4675 & 0.7664 & 0.7667 & 0.8324 & 0.6316 & 0.6982 & 0.4137 & 0.6024 & 0.8307 & 0.8215	\\
		ebank (TWAR) & 0.6857 & 0.7762 & 0.4091 & 0.7649 & 0.7576 & 0.8828 & 0.3544 & 0.6906 & 0.0000 & 0.0239 & 0.8668 & 0.8847	\\
		ebank (UM) & 0.6178 & 0.6541 & 0.3784 & 0.6396 & 0.6250 & 0.6892 & 0.4658 & 0.6073 & 0.3334 & 0.5099 & 0.6774 & 0.6786	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:prec_thr_0.5_transductive_mean}
\caption{Precision Results. \textcolor{red}{(hist-nre)} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.5973 & 0.5676 & 0.7010 & 0.5381 & 0.5712 & 0.7557 & 0.5327 & 0.5342 & 0.5606 & 0.6079 & 0.5598 & 0.5917	\\
		DyRep & 0.6101 & 0.5659 & 0.7183 & 0.5274 & 0.6138 & 0.8672 & 0.2673 & 0.5297 & 0.5421 & 0.6011 & 0.5449 & 0.5629	\\
		TGAT & 0.5546 & 0.5538 & 0.5490 & 0.4990 & 0.5128 & 0.7006 & 0.5122 & 0.5448 & 0.6209 & 0.6666 & 0.6114 & 0.5490	\\
		TGN & 0.5468 & 0.5594 & 0.7406 & 0.5006 & 0.5763 & 0.8209 & 0.5257 & 0.5311 & 0.5585 & 0.6613 & 0.5531 & 0.6583	\\
		CAWN & 0.4980 & 0.6150 & 0.4992 & 0.5031 & 0.4907 & 0.5368 & 0.5224 & 0.5069 & 0.7835 & 0.9570 & 0.5225 & 0.7553	\\
		\midrule
		ebank (RF) & 0.8523 & 0.8227 & 0.3982 & 0.7331 & 0.7404 & 0.8517 & 0.5865 & 0.8202 & 0.3210 & 0.3825 & 0.7826 & 0.6743	\\
		ebank (TWF) & 0.7847 & 0.7401 & 0.6975 & 0.7344 & 0.7047 & 0.7145 & 0.7797 & 0.7147 & 0.4461 & 0.7557 & 0.7481 & 0.7093	\\
		ebank (TWAR) & 0.9136 & 0.8125 & 0.8917 & 0.8161 & 0.8914 & 0.7968 & 0.9840 & 0.7647 & 0.9804 & 0.9923 & 0.8527 & 0.8666	\\
		ebank (UM) & 0.4943 & 0.5082 & 0.3359 & 0.5003 & 0.4840 & 0.5259 & 0.3941 & 0.4814 & 0.2705 & 0.4230 & 0.5192 & 0.5147	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:rec_thr_0.5_transductive_mean}
\caption{Recall Results. \textcolor{red}{(hist-nre)} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.8891 & 0.9353 & 0.8255 & 0.9210 & 0.8832 & 0.8379 & 0.1900 & 0.9371 & 0.9047 & 0.9796 & 0.8217 & 0.7693	\\
		DyRep & 0.8551 & 0.9375 & 0.8335 & 0.9785 & 0.8642 & 0.8605 & 0.1115 & 0.9339 & 0.9448 & 0.6747 & 0.6679 & 0.8259	\\
		TGAT & 0.8780 & 0.9361 & 0.7827 & 0.8180 & 0.8199 & 0.7208 & 0.8926 & 0.8474 & 0.6630 & 0.8083 & 0.6935 & 0.5379	\\
		TGN & 0.9333 & 0.9459 & 0.8383 & 0.9993 & 0.9401 & 0.9264 & 0.9301 & 0.9289 & 0.9417 & 0.9279 & 0.8065 & 0.8227	\\
		CAWN & 0.9915 & 0.9894 & 0.9984 & 0.9860 & 0.9800 & 1.0000 & 0.9768 & 0.9986 & 0.8344 & 0.6433 & 0.9462 & 0.6044	\\
		\midrule
		ebank (RF) & 0.6588 & 0.7279 & 0.1636 & 0.5932 & 0.5294 & 0.8671 & 0.3814 & 0.6225 & 0.2714 & 0.1574 & 0.5516 & 0.4839	\\
		ebank (TWF) & 0.7451 & 0.8344 & 0.3540 & 0.8041 & 0.8484 & 0.9973 & 0.5349 & 0.6881 & 0.4067 & 0.5198 & 0.9353 & 0.9797	\\
		ebank (TWAR) & 0.5526 & 0.7442 & 0.2702 & 0.7248 & 0.6764 & 0.9915 & 0.2228 & 0.6371 & 0.0000 & 0.0190 & 0.8836 & 0.9275	\\
		ebank (UM) & 0.8241 & 0.9178 & 0.4340 & 0.8870 & 0.8854 & 0.9997 & 0.5706 & 0.8239 & 0.4438 & 0.6440 & 0.9744 & 0.9956	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}











==> content/arXiv/103_app_induc_nre.tex.tex <==
\subsection{Adversarial Negative Edge Sampling: INDUC-NRE}

\begin{table*}
\label{tab:acc_thr_0.5_transductive_mean}
\caption{Accuracy Results. \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.5285 & 0.5920 & 0.6061 & 0.5084 & 0.5912 & 0.7734 & 0.4552 & 0.5560 & 0.6060 & 0.6862 & 0.6212 & 0.6674	\\
		DyRep & 0.5414 & 0.5929 & 0.5777 & 0.5044 & 0.6056 & 0.8546 & 0.5131 & 0.5504 & 0.5801 & 0.6457 & 0.5958 & 0.6431	\\
		TGAT & 0.6201 & 0.6517 & 0.5379 & 0.4989 & 0.5500 & 0.7237 & 0.5292 & 0.5966 & 0.6477 & 0.6865 & 0.5693 & 0.5085	\\
		TGN & 0.5577 & 0.5770 & 0.6754 & 0.5002 & 0.5806 & 0.8683 & 0.4989 & 0.5761 & 0.5883 & 0.7290 & 0.6330 & 0.7230	\\
		CAWN & 0.4984 & 0.7420 & 0.4994 & 0.5001 & 0.4904 & 0.5221 & 0.5240 & 0.5287 & 0.6965 & 0.7864 & 0.5683 & 0.6170	\\
		\midrule
		ebank (RF) & 0.8181 & 0.8595 & 0.4803 & 0.7738 & 0.7501 & 0.8735 & 0.5865 & 0.8110 & 0.6133 & 0.5194 & 0.7420 & 0.6680	\\
		ebank (TWF) & 0.4040 & 0.4280 & 0.1856 & 0.4084 & 0.5235 & 0.7743 & 0.2937 & 0.3791 & 0.5359 & 0.6853 & 0.5731 & 0.5766	\\
		ebank (TWAR) & 0.5880 & 0.5119 & 0.4191 & 0.4597 & 0.7259 & 0.8508 & 0.5792 & 0.4032 & 0.4924 & 0.4837 & 0.6382 & 0.7281	\\
		ebank (UM) & 0.4334 & 0.4665 & 0.2193 & 0.4457 & 0.5335 & 0.5947 & 0.3075 & 0.4445 & 0.4891 & 0.6003 & 0.5686 & 0.5556	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:ap_inherent_transductive_mean}
\caption{AP Results.  \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.6626 & 0.8411 & 0.6585 & 0.5991 & 0.5932 & 0.7168 & 0.4942 & 0.6817 & 0.4816 & 0.4503 & 0.5859 & 0.6661	\\
		DyRep & 0.6897 & 0.8542 & 0.6284 & 0.6295 & 0.6744 & 0.9201 & 0.5417 & 0.6496 & 0.5735 & 0.6399 & 0.6158 & 0.6437	\\
		TGAT & 0.8159 & 0.8793 & 0.5421 & 0.5001 & 0.5662 & 0.7872 & 0.6188 & 0.7006 & 0.6690 & 0.5797 & 0.5428 & 0.5120	\\
		TGN & 0.8656 & 0.8804 & 0.7696 & 0.6748 & 0.7036 & 0.9458 & 0.6932 & 0.6940 & 0.5220 & 0.5287 & 0.6336 & 0.7019	\\
		CAWN & 0.8585 & 0.9674 & 0.6615 & 0.7031 & 0.5720 & 0.5984 & 0.8342 & 0.6941 & 0.8464 & 0.8075 & 0.6669 & 0.7604	\\
		\midrule
		ebank (RF) & 0.8077 & 0.8552 & 0.4939 & 0.7551 & 0.7391 & 0.8287 & 0.5603 & 0.8108 & 0.6215 & 0.5172 & 0.7296 & 0.6464	\\
		ebank (TWF) & 0.4643 & 0.4692 & 0.4193 & 0.4606 & 0.5365 & 0.6904 & 0.4327 & 0.4667 & 0.5944 & 0.6454 & 0.5570 & 0.5450	\\
		ebank (TWAR) & 0.5764 & 0.5161 & 0.4860 & 0.4884 & 0.6793 & 0.7742 & 0.5734 & 0.4783 & 0.5000 & 0.5063 & 0.6001 & 0.6624	\\
		ebank (UM) & 0.4758 & 0.4861 & 0.4167 & 0.4754 & 0.5401 & 0.5525 & 0.4352 & 0.4905 & 0.5492 & 0.5617 & 0.5461 & 0.5306	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:au_pr_score_transductive_mean}
\caption{AU-PR Results. \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.6599 & 0.8406 & 0.6563 & 0.5963 & 0.5757 & 0.7138 & 0.4917 & 0.6792 & 0.4796 & 0.4485 & 0.5641 & 0.6618	\\
		DyRep & 0.6768 & 0.8536 & 0.6237 & 0.6235 & 0.6519 & 0.9184 & 0.5322 & 0.6474 & 0.5713 & 0.6369 & 0.5971 & 0.6399	\\
		TGAT & 0.8152 & 0.8789 & 0.5390 & 0.6486 & 0.5633 & 0.7859 & 0.6173 & 0.6985 & 0.6663 & 0.5768 & 0.5903 & 0.5086	\\
		TGN & 0.8652 & 0.8801 & 0.7687 & 0.6733 & 0.6912 & 0.9454 & 0.6923 & 0.6916 & 0.5194 & 0.5265 & 0.6306 & 0.6993	\\
		CAWN & 0.8565 & 0.9671 & 0.7578 & 0.7010 & 0.5582 & 0.5959 & 0.8292 & 0.8233 & 0.8440 & 0.8050 & 0.6615 & 0.7566	\\
		\midrule
		ebank (RF) & 0.8981 & 0.9259 & 0.5111 & 0.8616 & 0.8394 & 0.9057 & 0.6706 & 0.9052 & 0.5758 & 0.5498 & 0.8347 & 0.7534	\\
		ebank (TWF) & 0.6613 & 0.6899 & 0.4709 & 0.6753 & 0.7269 & 0.8448 & 0.5693 & 0.6444 & 0.5507 & 0.7635 & 0.7643 & 0.7672	\\
		ebank (TWAR) & 0.7049 & 0.6963 & 0.5315 & 0.6711 & 0.7968 & 0.8862 & 0.7064 & 0.6371 & 0.4324 & 0.2754 & 0.7770 & 0.8101	\\
		ebank (UM) & 0.6907 & 0.7218 & 0.5099 & 0.7074 & 0.7375 & 0.7762 & 0.5846 & 0.6991 & 0.5594 & 0.7050 & 0.7673 & 0.7642	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:auc_inherent_transductive_mean}
\caption{AU-ROC Results. \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.6568 & 0.8120 & 0.6651 & 0.5855 & 0.6347 & 0.8195 & 0.5495 & 0.6899 & 0.4986 & 0.4954 & 0.6396 & 0.7149	\\
		DyRep & 0.6657 & 0.8227 & 0.6346 & 0.6076 & 0.6801 & 0.9251 & 0.5405 & 0.6665 & 0.6263 & 0.7085 & 0.6304 & 0.6874	\\
		TGAT & 0.7862 & 0.8575 & 0.5513 & 0.4979 & 0.5784 & 0.8000 & 0.5876 & 0.6964 & 0.7074 & 0.6834 & 0.5766 & 0.5296	\\
		TGN & 0.8179 & 0.8464 & 0.7653 & 0.6483 & 0.7053 & 0.9479 & 0.6185 & 0.7034 & 0.5780 & 0.6425 & 0.6789 & 0.7661	\\
		CAWN & 0.8022 & 0.9575 & 0.5966 & 0.5862 & 0.4176 & 0.5007 & 0.7841 & 0.6768 & 0.7881 & 0.7241 & 0.5233 & 0.6693	\\
		\midrule
		ebank (RF) & 0.8181 & 0.8595 & 0.4803 & 0.7738 & 0.7501 & 0.8735 & 0.5865 & 0.8110 & 0.6133 & 0.5194 & 0.7420 & 0.6680	\\
		ebank (TWF) & 0.4040 & 0.4280 & 0.1856 & 0.4084 & 0.5235 & 0.7743 & 0.2937 & 0.3791 & 0.5359 & 0.6853 & 0.5731 & 0.5766	\\
		ebank (TWAR) & 0.5880 & 0.5119 & 0.4191 & 0.4597 & 0.7259 & 0.8508 & 0.5792 & 0.4032 & 0.4924 & 0.4837 & 0.6382 & 0.7281	\\
		ebank (UM) & 0.4334 & 0.4665 & 0.2193 & 0.4457 & 0.5335 & 0.5947 & 0.3075 & 0.4445 & 0.4891 & 0.6003 & 0.5686 & 0.5556	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}


\begin{table*}
\label{tab:f1_thr_0.5_transductive_mean}
\caption{F1-score Results. \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.6539 & 0.6969 & 0.6766 & 0.6489 & 0.6806 & 0.7851 & 0.2441 & 0.6819 & 0.6906 & 0.7570 & 0.6788 & 0.6582	\\
		DyRep & 0.6512 & 0.6979 & 0.6635 & 0.6636 & 0.6846 & 0.8539 & 0.1624 & 0.6782 & 0.6891 & 0.6183 & 0.6053 & 0.6675	\\
		TGAT & 0.6990 & 0.7294 & 0.6288 & 0.6069 & 0.6434 & 0.7211 & 0.6547 & 0.6785 & 0.6226 & 0.7193 & 0.5416 & 0.4174	\\
		TGN & 0.6797 & 0.6917 & 0.7209 & 0.6666 & 0.6924 & 0.8756 & 0.6502 & 0.6906 & 0.6919 & 0.7721 & 0.6811 & 0.7397	\\
		CAWN & 0.6635 & 0.8199 & 0.6658 & 0.6588 & 0.6539 & 0.6814 & 0.6716 & 0.6850 & 0.7091 & 0.6337 & 0.6929 & 0.5035	\\
		\midrule
		ebank (RF) & 0.7810 & 0.8375 & 0.2370 & 0.7149 & 0.6525 & 0.8706 & 0.4729 & 0.7572 & 0.3137 & 0.2377 & 0.6537 & 0.5729	\\
		ebank (TWF) & 0.5578 & 0.5942 & 0.3018 & 0.5752 & 0.6441 & 0.8159 & 0.4311 & 0.5292 & 0.3752 & 0.6095 & 0.6950 & 0.6991	\\
		ebank (TWAR) & 0.5802 & 0.6088 & 0.3217 & 0.5738 & 0.7026 & 0.8701 & 0.3397 & 0.5197 & 0.0000 & 0.0242 & 0.7172 & 0.7643	\\
		ebank (UM) & 0.5949 & 0.6334 & 0.3560 & 0.6151 & 0.6583 & 0.7116 & 0.4525 & 0.6027 & 0.3959 & 0.6129 & 0.6979 & 0.6920	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}



\begin{table*}
\label{tab:prec_thr_0.5_transductive_mean}
\caption{Precision Results. \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.5182 & 0.5561 & 0.5744 & 0.5062 & 0.5561 & 0.7472 & 0.3732 & 0.5404 & 0.5619 & 0.6174 & 0.5842 & 0.5972	\\
		DyRep & 0.5275 & 0.5566 & 0.5532 & 0.5025 & 0.5746 & 0.8539 & 0.5032 & 0.5366 & 0.5443 & 0.6178 & 0.5764 & 0.5744	\\
		TGAT & 0.5817 & 0.5980 & 0.5255 & 0.4990 & 0.5324 & 0.7242 & 0.5179 & 0.5677 & 0.6163 & 0.6499 & 0.6456 & 0.4774	\\
		TGN & 0.5358 & 0.5460 & 0.6355 & 0.5001 & 0.5520 & 0.8312 & 0.5010 & 0.5551 & 0.5497 & 0.6626 & 0.5965 & 0.6913	\\
		CAWN & 0.4984 & 0.7399 & 0.4994 & 0.5045 & 0.4908 & 0.5221 & 0.5226 & 0.5278 & 0.7166 & 0.9259 & 0.5698 & 0.7688	\\
		\midrule
		ebank (RF) & 0.9668 & 0.9880 & 0.4404 & 0.9267 & 0.9141 & 0.8779 & 0.6504 & 0.9992 & 0.5159 & 0.5209 & 0.8937 & 0.7649	\\
		ebank (TWF) & 0.4500 & 0.4627 & 0.2648 & 0.4486 & 0.5296 & 0.6909 & 0.3712 & 0.4447 & 0.3980 & 0.7671 & 0.5609 & 0.5445	\\
		ebank (TWAR) & 0.6334 & 0.5206 & 0.4279 & 0.4797 & 0.7554 & 0.7767 & 0.8014 & 0.4556 & 0.3647 & 0.0413 & 0.6122 & 0.6564	\\
		ebank (UM) & 0.4694 & 0.4847 & 0.3028 & 0.4713 & 0.5323 & 0.5525 & 0.3839 & 0.4864 & 0.3969 & 0.5879 & 0.5474 & 0.5307	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}



\begin{table*}
\label{tab:rec_thr_0.5_transductive_mean}
\caption{Recall Results. \textcolor{red}{induc-nre} }
\resizebox{\linewidth}{!}{
	\begin{tabular}{c c c c c c c c | c c c c c}
	\toprule
		Method & wikipedia & reddit & mooc & lastfm & enron & socialevolve & uci & SkyNet & canVote & LegisEdgelist & UNtrade & UNvote	\\
	\midrule
		JODIE & 0.8891 & 0.9353 & 0.8255 & 0.9210 & 0.8832 & 0.8379 & 0.1900 & 0.9371 & 0.9047 & 0.9796 & 0.8217 & 0.7693	\\
		DyRep & 0.8551 & 0.9375 & 0.8335 & 0.9785 & 0.8642 & 0.8605 & 0.1115 & 0.9339 & 0.9448 & 0.6747 & 0.6679 & 0.8259	\\
		TGAT & 0.8793 & 0.9363 & 0.7837 & 0.8184 & 0.8189 & 0.7206 & 0.8915 & 0.8472 & 0.6625 & 0.8092 & 0.6939 & 0.5379	\\
		TGN & 0.9333 & 0.9459 & 0.8383 & 0.9993 & 0.9401 & 0.9264 & 0.9301 & 0.9289 & 0.9417 & 0.9279 & 0.8065 & 0.8227	\\
		CAWN & 0.9933 & 0.9886 & 0.9985 & 0.9857 & 0.9799 & 1.0000 & 0.9755 & 0.9986 & 0.8301 & 0.6432 & 0.9483 & 0.6039	\\
		\midrule
		ebank (RF) & 0.6588 & 0.7279 & 0.1636 & 0.5932 & 0.5294 & 0.8671 & 0.3814 & 0.6225 & 0.2714 & 0.1574 & 0.5516 & 0.4839	\\
		ebank (TWF) & 0.7451 & 0.8344 & 0.3540 & 0.8041 & 0.8484 & 0.9973 & 0.5349 & 0.6881 & 0.4067 & 0.5198 & 0.9353 & 0.9797	\\
		ebank (TWAR) & 0.5526 & 0.7442 & 0.2702 & 0.7248 & 0.6764 & 0.9915 & 0.2228 & 0.6371 & 0.0000 & 0.0190 & 0.8836 & 0.9275	\\
		ebank (UM) & 0.8241 & 0.9178 & 0.4340 & 0.8870 & 0.8854 & 0.9997 & 0.5706 & 0.8239 & 0.4438 & 0.6440 & 0.9744 & 0.9956	\\
	\bottomrule
	\end{tabular}
	}
\end{table*}








==> content/arXiv/110_app.tex <==
\clearpage
 \onecolumn 
 
\section{Broader Impact} 
\label{app:impact}

%https://neurips.cc/public/EthicsGuidelines

\textbf{Impact on Dynamic Graph ML Research}

\textbf{Impact on Different Applications}

\textbf{Potential Negative Impact}
 
 
 
\section{Limitations} 
\label{app:limit}
Not enough datasets, the benchmark setup is limited to link prediction,

In future work, we aim to synthesize insights here into concise measurements that summarize the difficulty of different datasets. We will also expand this work to temporal node classification, another key task. Finally, we hope to apply our tools to produce novel and effective DGNN models.



\section{Computing Resources}
\label{sec:computing_resources}

\textcolor{red}{The total compute and the type of resources used...}
